ZoomLynx: Learning to Zoom In on What Matters

Active reasoning matters. High-resolution visual tasks require models to seek local evidence and adapt their next move to what they observe. Yet base vision-language models may repeat uninformative zoom calls without correcting localization or recognizing when to stop. Existing approaches compensate for localization errors through multi-round search, region refinement, and feedback verification, increasing inference cost. Effective visual reasoning therefore calls for a structured observation process in which reasoning guides evidence acquisition and actual observations shape subsequent decisions. We introduce ZoomLynx, a visual reasoning agent named for the lynx's keen sight and agility. Using a single zoom tool, ZoomLynx organizes evidence acquisition around three explicit decisions: When to inspect, Where to zoom, and when to Stop. To supervise these decisions, we develop a data pipeline that converts real tool interactions into structured training trajectories tailored to the model's current capabilities. Drawing on both successful and failed observations, the pipeline provides complementary supervision for selective inspection, recovery, and stopping. We learn observation policies from these trajectories through Selective Zoom Training and subsequent preference optimization. We further introduce Aperture-580, a benchmark for a more comprehensive evaluation of active visual reasoning. On ZoomBench and V*Bench, the 4B GSPO model scores above GPT-5.5 and Gemini-3.1-pro in their direct-answer settings. Behavioral analyses show reduced unnecessary calls and improved evidence localization. These results demonstrate the value of coupling structured observation data with policy learning to enable purposeful zooming for active visual reasoning.

==> compile_compat.tex <==
\makeatletter
\@ifpackagelater{microtype}{2025/02/12}{}{%
\def\MT@setup@expansion{%
  \ifnum\pdfoutput<\@ne
    \ifMT@opt@expansion
    \else
      \MT@expansionfalse
    \fi
  \fi
  \ifMT@expansion
    \ifnum\MT@stretch=\m@ne
      \let\MT@stretch\MT@stretch@default
    \fi
    \ifnum\MT@shrink=\m@ne
      \let\MT@shrink\MT@stretch
    \fi
    \ifnum\MT@step=\m@ne
    \MT@requires@pdftex6{%
      \def\MT@step{1 }%
    }{%
      \ifnum\MT@stretch>\MT@shrink
        \ifnum\MT@shrink=\z@
          \@tempcnta=\MT@stretch
        \else
          \@tempcnta=\MT@shrink
        \fi
      \else
        \ifnum\MT@stretch=\z@
          \@tempcnta=\MT@shrink
        \else
          \@tempcnta=\MT@stretch
        \fi
      \fi
      \divide\@tempcnta 5\relax
      \ifnum\@tempcnta=\z@ \@tempcnta=\@ne \fi
      \edef\MT@step{\number\@tempcnta\space}%
    }%
    \fi
    \ifnum\MT@step=\z@
      \MT@warning@nl{The expansion step cannot be set to zero.\MessageBreak
          Setting it to one}%
      \def\MT@step{1 }%
    \fi
    \let\MT@auto\@empty
    \ifMT@auto
      \MT@requires@pdftex4{%
        \ifnum\pdfoutput<\@ne
          \ifMT@opt@auto
            \MT@error{%
              Automatic font expansion only works for PDF output.\MessageBreak
              However, you are creating a DVI file}
             {If you have created expanded fonts instances, remove `auto' from%
              \MessageBreak the package options. Otherwise, you have to switch
              off expansion\MessageBreak completely.}%
          \fi
          \MT@autofalse
        \else
          \def\MT@auto{autoexpand}%
        \fi
      }{%
        \MT@error{%
          The pdftex version you are using is too old for\MessageBreak
          automatic font expansion}%
         {If you have created expanded fonts instances, remove `auto' from\MessageBreak
          the package options. Otherwise, you have to switch off expansion\MessageBreak
          completely, or upgrade pdftex to version 1.20 or newer.}%
        \MT@autofalse
        \def\MT@auto{1000 }%
      }%
    \else
      \MT@requires@pdftex4\relax{%
        \def\MT@auto{1000 }%
      }%
    \fi
    \ifMT@selected
      \let\MT@set@ex@codes\MT@set@ex@codes@s
    \else
      \let\MT@set@ex@codes\MT@set@ex@codes@n
    \fi
    \ifnum\MT@stretch=\z@
      \ifnum\MT@shrink=\z@
        \MT@warning@nl{%
          Both the stretch and shrink limit are set to zero.\MessageBreak
          Disabling font expansion}%
        \MT@expansionfalse
      \fi
    \fi
  \fi
  \ifMT@expansion
    \edef\MT@active@features{\MT@active@features,ex}%
    \MT@adjustspacing\MT@ex@level
    \MT@info@nl{\ifMT@auto A\else Non-a\fi utomatic font expansion enabled
                (level \number\MT@ex@level),\MessageBreak
                stretch: \number\MT@stretch, shrink: \number\MT@shrink,
                step: \number\MT@step, \ifMT@selected\else non-\fi selected}%
    \def\MT@check@step##1{%
      \@tempcnta=\csname MT@##1\endcsname
      \divide\@tempcnta \MT@step
      \multiply\@tempcnta \MT@step
      \ifnum\@tempcnta=\csname MT@##1\endcsname\else
        \MT@warning@nl{The ##1 amount is not a multiple of step.\MessageBreak
                       The effective maximum ##1 is \the\@tempcnta\space
                       (step \number\MT@step)}%
      \fi
    }%
    \MT@check@step{stretch}%
    \MT@check@step{shrink}%
    \MT@check@active@set{ex}%
    \MT@ifdefined@n@TF{showhyphens }{%
      \MT@exp@cs\patchcmd{showhyphens }{\color@begingroup}{\color@begingroup\pdfadjustspacing\z@}
        {\MT@info@nl{Patching command `\string\showhyphens'}}
        {\MT@warning@nl{Unable to patch command `\string\showhyphens'}}%
    }{%
      \CheckCommand*\showhyphens[1]{\setbox0\vbox{\color@begingroup
        \everypar{}\parfillskip\z@skip\hsize\maxdimen\normalfont
        \pretolerance\m@ne\tolerance\m@ne\hbadness\z@\showboxdepth\z@\ ##1\color@endgroup}}
      \gdef\showhyphens##1{\setbox0\vbox{\color@begingroup\pdfadjustspacing\z@
        \everypar{}\parfillskip\z@skip\hsize\maxdimen\normalfont
        \pretolerance\m@ne\tolerance\m@ne\hbadness\z@\showboxdepth\z@\ ##1\color@endgroup}}%
    }%
  \else
    \let\MT@expansion\relax
    \MT@info@nl{No font expansion}%
  \fi
}
}
\makeatother
\DeclareFontShape{T1}{papersans}{b}{it}{<-> s * [0.88] assets/papersans}{}

